OpenMLDB: A Real-Time Relational Data Feature Computation System for Online ML

Efficient and consistent feature computation is crucial for a wide range of online ML applications. Typically, feature computation is divided into two distinct phases, i.e., offline stage for model training and online stage for model serving. These phases often rely on execution engines with different interface languages and function implementations, causing significant inconsistencies. Moreover, many online ML features involve complex time-series computations (e.g., functions over varied-length table windows) that differ from standard streaming and analytical queries. Existing data processing systems (e.g., Spark, Flink, DuckDB) often incur multi-second latencies for these computations, making them unsuitable for real-time online ML applications that demand timely feature updates. This paper presents OpenMLDB, a feature computation system deployed in 4Paradigm's SageOne platform and over 100 real scenarios. Technically, OpenMLDB first employs a unified query plan generator for consistent computation results across the offline and online stages, significantly reducing feature deployment overhead. Second, OpenMLDB provides an online execution engine that resolves performance bottlenecks caused by long window computations (via pre-aggregation) and multi-table window unions (via data self-adjusting). It also provides a high-performance offline execution engine with window parallel optimization and time-aware data skew resolving. Third, OpenMLDB features a compact data format and stream-focused indexing to maximize memory usage and accelerate data access. Evaluations in testing and real workloads reveal significant performance improvements and resource savings compared to the baseline systems. The open community of OpenMLDB now has over 150 contributors and gained 1.6k stars on GitHub.

==> 2_motivation.tex <==

\vspace{-.25em}
\section{Background and motivation}\label{sec:mot}





\iffalse
%In this section, we introduce database dialects and incompatibility issues caused by migrating queries across database dialects (Section~\ref{subsec:incompatible}), formalize the definition of dialect translation (Section~\ref{subsec:def}), and review the limitations of existing translation methods (Section~\ref{subsec:def-problems}).

% In this section, we first introduce Database Dialect \zw{?}, then review typical dialect incompatibility issues, and finally formalize the definition of how Database Dialect Translation resolves these issues.

\subsection{Database Dialect and Incompatibility}
\label{subsec:incompatible}

\bfit{Database Dialect} refers to the specific implementation of SQL standards in a database. Syntax differences between database dialects can cause \textit{incompatibility issues},  where a SQL query written for one database may fail to execute correctly on another. Incompatibilities typically arise from differences in the following five aspects.

{\it (1) Syntax Rules:} Databases may use distinct syntax rules for common operations such as column and table annotations and the definitions about join and data manipulation. For example, a subquery without an alias is allowed in Oracle, while MySQL requires that each subquery must be assigned an alias.

\begin{sloppypar}
{\it (2) Keywords:} Databases contain a set of reserved keywords to support different operations. For example, PostgreSQL has the keyword \textsf{FULL OUTER JOIN} for fetching all the rows from joined tables, while MySQL can only obtain the same functionality combined with the two keywords \textsf{LEFT} and \textsf{RIGHT OUTER JOIN}. Besides, the keyword \textsf{NULL LAST} in PostgreSQL specifies the order of null values, which is also not supported in MySQL.
\end{sloppypar}

\begin{sloppypar}
{\it (3) Functions and Operators:} Databases implement a series of (customized) functions and operators. For example, MySQL develops a function ``LAST\_DAY()'' to return the last day of a month, while PostgreSQL can utilize the ``DATE\_TRUNC()'' function and ``+'' and ``-'' arithmetic operators to achieve the same functionality.
\end{sloppypar}
% over an arithmetic calculation by
% Each database system has its own set of functions and reserved keywords. A function available in one database dialect might be unsupported or have a different name in another. For instance, transferring ``SELECT NOW()'' from MySQL to Oracle triggers a warning ``NOW() is unsupported''.

\begin{sloppypar}
{\it (4) Data Types:} Databases may have different names for the same or similar data types. For example, MySQL leverages \textsf{DATETIME} to annotate the date type, while Oracle adopts \textsf{DATE} and \textsf{TIMESTAMP}.  
\end{sloppypar}
% For example, when migrating a PostgreSQL query using the JSONB data type to a version before 9.4, it triggers a warning that indicates JSONB is unsupported and we should use JSON instead.

%Even within the same database, different versions may introduce new features or deprecate old ones, causing a query to fail or behave unexpectedly across versions. For instance, PostgreSQL’s {\it jsonb} data type was introduced in version 9.4, so queries using {\it jsonb} would fail in earlier versions. \zw{Example: Oracle 11g: ROWNUM, Oracle 19c: FETCH FIRST n ROW ONLY}

\begin{sloppypar}
{\it (5) Others:} Databases may handle constraints (e.g., foreign keys, unique columns) and system settings differently. For instance, MySQL on Linux is case-sensitive by default (with lower\_case\_table\_names=0), while PostgreSQL usually converts table and column names to lowercase, making it case-insensitive.
\end{sloppypar}

Note that we use \emph{syntax elements} to represent keywords, function,s and operators in the following sections without ambiguity.

% {\it (4) Constraints and Indexing:} Databases handle constraints (e.g., foreign keys, unique columns) and indexing mechanisms differently, which can lead to incompatibilities during dialect translation. For instance, migrating a MySQL table definition statement with FOREIGN KEY constraints to Oracle triggers a warning that \zxh{add}.

%Note that in this paper we focus on queries involving common functions across mainstream databases. Advanced functions, such as user-defined functions (UDFs) and stored procedures, are considered as future work. 

\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{figures/dialect_intro_error_v2.pdf}
  % {figures/motivation.png}
  \vspace{-1.75em}
  \caption{Error Distribution of Dialect Translation from PostgreSQL to MySQL {for TPC-DS queries} (\emph{Others} denote the queries that yield different results due to the inner difference of databases, e.g., the precision of numeric values).}
  \label{fig: mot}
  \vspace{-1em}
\end{figure}

\subsection{Database Dialect Translation}
\label{subsec:def}

\bfit{Database Dialect Translation} refers to translating a query that causes incompatibility issues by following the standards of target database dialect to ensure compatibility and {\it equivalent functionality} when executing in the target database system.

\begin{definition}[Functional Equivalence]
A query operation \( q_i^T \), which is an implementation of syntax \( S_i^T \), in database \( D^T \) is \textit{functionally equivalent} to a query operation \( q_i^O \) in database \( D^O \) if it produces the same execution results or has the same effect as \( q_i^O \).
\end{definition}

% satisfies one of the following conditions: (1) If \( O_i^T \) is a Data Manipulation Language (DML) operation, it produces the same execution results as \( O_i^O \); (2) If \( O_i^T \) is a Data Definition Language (DDL) operation, it has the same effect on database \( D^T \) as \( O_i^O \) has on \( D^O \).

%\zw{?}

\iffalse
\begin{example}
In PostgreSQL, the operation \textsf{`Romantic' \textbar\textbar\ `-Movie'} concatenates the two strings, which is functionally equivalent to \textsf{CONCAT(`Romantic', `-Movie')} in MySQL.
\end{example}
\fi

\begin{example}
In PostgreSQL, the operation \textsf{CONCAT(`hello', NULL)} returns \textsf{``hello''}, while in MySQL, \textsf{CONCAT(`hello', NULL)} returns \textsf{NULL}. These operations are not functionally equivalent. To achieve the same result, the MySQL operation should include a conditional expression, such as \textsf{CASE \dots WHEN}.
\end{example}

\begin{example}
Within the \textsf{CREATE} clause, \textsf{NUMERIC}(10, 2) in PostgreSQL is equivalent to \textsf{NUMBER}(10, 2) in  Oracle, both defining a numeric column with up to 10 digits, including 2 decimal places.
%In PostgreSQL,  is functionally equivalent to NUMBER(10, 2) in Oracle \zw{specifying the type if the column in \textsf{CREATE} clause}, as both store numeric values with up to 10 total digits, including 2 decimal places.
\end{example}

\begin{definition}[Database Dialect Translation]
Given a query \( Q^O \) written in a source database dialect, \( Q^O \) is composed of one or more operations \( \{q_i^O\} \). \textit{Database Dialect Translation} refers to the process of mapping each operation \( q_i^O \) to one or more functionally equivalent operations in the target database dialect. The translated query \( Q^T \) must (1) strictly follow the target dialect syntax \( S^T \) and (2) maintain functional equivalence to \( Q^O \).
\end{definition}

\begin{example}
As shown in Figure~\ref{fig:intro}, translating a PostgreSQL query that {\it retrieves the names of people younger than 70} into an equivalent MySQL-compatible query requires separately translating both the \textsf{CAST} and \textsf{EXTRACT} operations. Specifically, we first resolve the data type incompatibility by replacing \textsf{TEXT} with \textsf{CHAR} in the \textsf{CAST} operation. Then we modify the \textsf{EXTRACT} operation to account for MySQL's lack of support for the \textsf{AGE} function.
\end{example}

Note that dialect translation and query rewrite~\cite{WeTune,llm4rewrite} are two different problems. (1) \textit{Query Rewrite} transforms queries under the same dialect, while \textit{Dialect Translation} converts between different dialects. (2) \textit{Query Rewrite} modifies query structures for better performance; while \textit{Dialect Translation} adjusts queries to match another dialect's syntax to resolve incompatibilities. 

In this paper, we research how to process queries into normalized operations with lower translation complexity (see Section~\ref{sec: processor}), how to match equivalent syntax elements in the target database dialect (see Section~\ref{sec:embed}), and how to accurately translate queries from the local operation level to the global query level (see Section~\ref{sec: translate}).

%resolving the query incompatibility problems by converting queries from one database dialect to another, while ensuring functional equivalence.
%by transforming a query written for an origin database into a functionally equivalent query that is valid in the target database.


\iffalse
\begin{definition}[Functional Equivalence]
An operation \( O_i^T \) in database $D^T$ is functionally equivalent to the operation \( O_i^O \) in the database $D^O$ if the output produced by \( O_i^T \) achieves the same execution results (when \( O_i^T \) is a DML operation) or have the same effects (when \( O_i^T \) is a DDL operation) to the database as \( O_i^O \) .
\end{definition}

\begin{definition}[Functional Equivalence]
An operation \( O_i^T \) in database \( D^T \) is {\it functionally equivalent} to an operation \( O_i^O \) in database \( D^O \) if and only if:
\begin{itemize}
    \item For Data Manipulation Language (DML) operations, \( O_i^T \) produces the same execution results as \( O_i^O \).
    \item For Data Definition Language (DDL) operations, \( O_i^T \) has the same effects on the database as \( O_i^O \).
\end{itemize}
\end{definition}
\fi

% string concatenation is performed using the `||' operator (e.g., `text' || `-book'), whereas in MySQL, the CONCAT function is used (e.g., CONCAT(text, `-book')). They yield the same result and are functionally equivalent.

%Note functionally equivalent queries across different databases may produce different results due to implementation differences (e.g., handling NULL values), requiring human validation for equivalence checking.


% Functional equivalence refers to the property where two distinct operations, applied in different database systems, produce the same outcome or effect. Specifically, in the context of query dialect translation, a


% transform an input query from origin database to resolve the incompatibility problems and successfully execute and output the correct result on the target database (i.e., achieving the intent of the input query).

% transform \( Q_O \) into a query \( Q_T \) that is valid in the target database. The transformation should ensure that  %This process guarantees that the translated query can execute successfully on the target database while preserving the same results of the original query.

%\zw{???Note we focus on queries that are composed of common functions shared by main-stream databases, and only the syntax of the same function can be different across databases. We explain how to process queries with composite functions in Section~\ref{sec:normalize}. Besides, advanced functions like UDF and storage procedure as future work.}

%If a composite function in the query can be converted into atomic operators (e.g., \zxh{add}), we preprocess the query to ensure no composite functions exist, which can be in favor of translating across databases. Besides, we take advanced functions like UDF and storage procedure as future work. %(3) Caused by implementations of different databases (e.g., the processing of NULL values), even the semantic-equivalent queries on different can output different results. Thus, for equivalence checking, we also need to examine by humans after checking the results.


\iffalse
For instance, consider the following query in PostgreSQL (the origin database):

\begin{verbatim}
SELECT CAST(DATE\_TRUNC('MONTH', CURRENT_DATE) + 
\end{verbatim}

\begin{verbatim}
INTERVAL '1 MONTH' - INTERVAL '1 DAY' AS DATE) AS result;
\end{verbatim}


This query returns the last day of the current month by truncating the current date to the start of the month, adding one month, and then subtracting one day. If we want to translate this query into a dialect for MySQL (the target database), the transformation would involve replacing the PostgreSQL-specific operators and functions with MySQL equivalents. For example, ``\textsf{DATE\_TRUNC()}'' does not exist in MySQL, and ``INTERVAL'' handling may slightly differ. \zxh{add}
\fi



\vspace{-.75em}
\subsection{Limitations of Existing Methods}
\label{subsec:def-problems}

To better understand the limitations of existing methods and design our system, we conducted a preliminary experiment (migrating TPC-DS queries from PostgreSQL to MySQL) that reveals the problems of SQLGlot~\cite{sqlglot}, \gpt, and Llama3.1~\cite{llama31} in dialect translation. As shown in Figure~\ref{fig: mot}, we have three observations.


\begin{sloppypar}
%\noindent \textbf{(Observation 1) Short Translation Query Operation over Lengthy Complex Queries.} Our first observation is that query operations require further translation only occupies small query parts in the lengthy TPC-DS template queries. Specifically, the number of the words in the experimented template queries is \zw{x} on average, while we notice that only the ROLLUP expressions for most \zw{y} template queries require translation (i.e., {GROUP BY ROLLUP(}col\_list{)} $\rightarrow$ {GROUP BY} col\_list {WITH ROLLUP}). This observation motivates us that translation typically occurs over the certain query operations since it needs to maintain the functionality equivalence of these operations across dialects. Accordingly, the translation can be operated at the local query operation level without the need of the whole input query and we can alleviate the translation effort by keeping the rest equivalent query operations unchanged.
\noindent \textbf{(Observation 1) Translation Affects Only Small Portions of Lengthy Complex Queries.}
Our first observation is that the query operations requiring translation occupy only small parts of the lengthy TPC-DS template queries.
Specifically, the number of words in the experimented template queries that require translation is {131} on average, while we notice that only the \textsf{ROLLUP} expressions in most of the template queries require translation (i.e., \textsf{GROUP BY ROLLUP(}col\_list\textsf{)} $\rightarrow$ \textsf{GROUP BY} col\_list \textsf{WITH ROLLUP}).
This observation motivates us to \textit{focus translation efforts on certain query operations that require functional equivalence across dialects}.
%Accordingly, the translation can be performed at the local query operation level without the need for the whole input query, and we can alleviate the translation effort by keeping the rest of the equivalent query operations unchanged.
\end{sloppypar}

\noindent \textbf{(Observation 2) Failure Due to Lack of Translation Rules and Knowledge.}
As shown in Figure~\ref{fig: mot}, \textsf{ROLLUP} and \textsf{FULL OUTER JOIN} account for a large proportion of translation failures.
Specifically, SQLGlot, \gpt, and Llama3.1 incur translation errors, i.e., {40.74\%, 29.63\% and 29.63\%} respectively, because they fail to handle the translation of \textsf{ROLLUP} and \textsf{FULL OUTER JOIN}.
This indicates that {\it existing rule-based translators lack certain translation rules, and LLMs are unaware of functionally equivalent specifications}, both of which are crucial for successful translation.

\noindent \textbf{(Observation 3) Error-Prone Characteristics of LLMs.}
We observe that LLMs are prone to making mistakes due to the hallucination problem.
Specifically, both \gpt and Llama3.1 might rename columns to ones that do not exist in the database (e.g., mistakenly changing ``\texttt{ca\_state}'' to ``\texttt{ca.state}'' based on their semantic understanding).
Furthermore, Llama3.1 makes syntax mistakes by appending the \textsf{SELECT} clause into the \textsf{WITH} clause as the last common table expression called ``\textsf{final\_result}'', which leads to the absence of a \textsf{SELECT} clause. It indicates {\it the necessity of enhancing the reliability of LLMs when applied in dialect translation with strict grammar requirements}.

%  or ``\texttt{returns}'' to ``\texttt{returns\_amt}''
% Since 72 out of the 99 template queries written in PostgreSQL can be directly executed over MySQL without any further translation, we experiment with the rest 27 queries.


\iffalse

\noindent \textbf{(Observation 3) Error-Prone Characteristics of \llms.}
We observe that \llms are likely to make mistakes due to the hallucination problem.
Specifically, both \gpt and Llama3.1 might rename the columns to the ones that do not exist in the database (i.e., mistakenly changing the name ``ca\_state'' into ``ca.state'' or ``returns'' into ``returns\_amt'' based on their semantic understanding).
Furthermore, Llama3.1 makes syntax mistakes by appending the SELECT clause into the WITH clause as the last common table expressions called ``\textsf{final\_result''}, which leads to the absence of a SELECT clause.
All of these indicate the necessity of enhancing the reliability of \llm by preprocessing the queries or other techniques when applied to dialect translation with strict grammar requirements.



Figure~\ref{fig:errors} shows the distribution of translation failure for rule-based engines and \llms, which reveals three main problems.

\hi{Hallucination Problem.} Some functions available in the source dialect are not supported by the target dialect. For instance, the PostgreSQL query \textsf{``CREATE TABLE a (LIKE b)''} copies the schema of table \texttt{b}, but MySQL does not support this syntax. In such cases, LLM generates non-existent functions, leading to translation failures. Meanwhile, caused by rule bugs, the translation engines also have a similar ``Hallucination Problem'', i.e., translating into unsupported functions. For instance, SQLGlot employs the \textsf{STR\_POSITION} function in an Oracle query, which does not exist in the Oracle dialect.


\hi{Ignoring Minor Differences.} LLM easily omits some subtle but important differences between the source and target dialects, leading to dialect translation failures, such as:

{\it (1) Data Types:} Variations in data type precision and naming, such as \textsf{DECIMAL} in MySQL versus \textsf{NUMERIC} in PostgreSQL.

{\it (2) Keywords:} For instance, in the PostgreSQL query \textsf{``SELECT * FROM employee ORDER BY salary ASC NULLS FIRST''}, it uses \textsf{NULLS FIRST} to sort the null values first, which GPT-4 ignores and causes different query results. 

{\it (3) Quotes:} For instance, MySQL uses \textsf{JSON\_UNQUOTE()}, while PostgreSQL uses \textsf{->>} for unquoting JSON values. 

{\it (4) Time Zones:} For instance, MySQL adjusts timestamps based on system time zones automatically, whereas PostgreSQL provides explicit control with \textsf{TIMESTAMP \dots TIME ZONE}. 

{\it (5) NULL Operand:} Differences in handling {null} values. For instance, \textsf{``IS NOT DISTINCT FROM''} in PostgreSQL includes rows with null values. In MySQL, the equivalent functionality is achieved using a null-safe equality operator like <=>.

\begin{sloppypar}
\hi{Model Misunderstanding.} LLM does not have a precise semantic understanding of some functions, causing failures like improper function usage. For instance, the built-in function \textsf{TO\_TIMESTAMP} in PostgreSQL converts Unix timestamps to date-time values, whereas the equivalent function in MySQL is  \textsf{FROM\_UNIXTIME}. However, \llm incorrectly uses \textsf{UNIX\_TIMESTAMP}. Similarly, the translation engine SQLines~\cite{sqlines} converts \textsf{TO\_TIMESTAMP} into CAST(... AS DATETIME) in MySQL, which is inequivalent to Unix timestamps.
\end{sloppypar}

\fi

\iffalse
\begin{sloppypar}
(4) {\textbf{Failure in Complex Calculations:}} Present in \emph{xx\%} of LLM translations compared to \emph{xxx\%} in rule engines. For example, calculating the last day of the current month in PostgreSQL using \emph{``CAST(DATE\_TRUNC('MONTH', CURRENT\_TIMESTAMP) + INTERVAL '1 MONTH' - INTERVAL '1 DAY' AS DATE)''} can be simplified in MySQL with \emph{LAST\_DAY(CURDATE())}, where \llm fails.
\end{sloppypar}


In summary, translation engines fail to translate due to limited rule coverage or some incorrect rules. LLM-based translation, suffers from the hallucination problem, has difficulty capturing the subtle nuances across different database dialects, and frequently misinterprets the intended functionality of operations. These limitations hinder the accuracy and reliability of dialect translation.

As shown in Figure~\ref{fig:errors}, traditional rule engines and \llms have their own problems in dialect translation. First, rule engines demonstrated errors across various categories: omission of keywords (\textbf{less than xx\%}), inaccurate handling of unsupported functions (\textbf{xx\%}), version incompatibility (\textbf{xxx\%}). 

\llms can resolve some of the errors (e.g., xxx), but also made many mistakes, including: (1) Omission of keywords (\textbf{xxx\%}). For instance, \llms often omitted critical operations like \emph{NULLS FIRST} in \emph{ORDER BY} statements. (2) Inaccurate handling of unsupported functions (\textbf{xxx\%}).  For instance, \emph{TO\_TIMESTAMP} in PostgreSQL is  equivalent to \emph{FROM\_UNIXTIME} in MySQL. However, \llm does not understand the function and uses a wrong function \emph{UNIX\_TIMESTAMP}. (3) 

\subsubsection{Rule-based Dialect Translation}

As discussed above, rule-based dialect translation has problems like missing translations, incorrect translations, and version incompatibility. And so they merely translate fewer than xxx\% queriies (Figure~\ref{fig:errors}).

\subsubsection{\llm-based Dialect Translation}

We investigated \zxh{add} typical dialect translation cases. As shown in Figure~\ref{fig:errors}, we find origin \llms have relatively poor accuracy in dialect translation. The main problems are as follows:

\zw{(summary -- update by fig2)}

\underline{\bfit{1. Omit Certain Keywords:}} For instance, for the query \emph{``SELECT * FROM employee ORDER BY salary ASC NULLS FIRST''} in PostgreSQL, the \emph{NULLS FIRST} keyword ensures the result rows with NULL values appear first. However, \llm may omit the keyword and cause the translated query non-equivalent.

\underline{\bfit{2. Lack Function Support:}} For instance, although PostgreSQL supports queries like \emph{``CREATE TABLE a (LIKE b)''}, which copies the schema of table b for table a, databases like MySQL do not own such function. However, \llm may fabricate a query with some non-existent syntax, rather than directly outputs ``Not Supported''.

\underline{\bfit{3. Use Wrong Function:}} For instance, \emph{TO\_TIMESTAMP} in PostgreSQL means converting the Unix timestamp into human-readable date-time values. The correct equivalent function in MySQL is \emph{FROM\_UNIXTIME}. However, \llm may do not understand the function and use a wrong function like ``UNIX\_TIMESTAMP''.

\begin{sloppypar}
\underline{\bfit{4. Fail to translate complex calculations.}} Some aggregations involve complex calculations and \llms may fail to understand the meaning and translate into wrong ones. For instance, in PostgreSQL, \emph{``CAST(DATE\_TRUNC('MONTH', CAST(CURRENT\_TIMESTAMP AS DATE)) + INTERVAL '1 MONTH' - INTERVAL '1 DAY' AS DATE)''} computes the last day of the current month. When translating into MySQL query, we can simply utilize the \emph{LAST\_DAY} function, which \llm cannot match and give the wrong translation.
\end{sloppypar}

\underline{\bfit{5. Ignore Minor Differences:}} \llms may not take care of many details when translating queries, such as: 

{\it (1) Quotes:} MySQL uses \emph{JSON\_UNQUOTE()} to remove quotes from JSON values. PostgreSQL uses ``\texttt{->>}'' for similar behavior. 

{\it (2) Time Zones:} MySQL automatically adjusts timestamps based on system time zones. PostgreSQL offers explicit control with \emph{TIMESTAMP WITH/WITHOUT TIME ZONE}. Ensure consistent time zone handling when translating. 

{\it (3) NULL Operand Behavior:} MySQL and PostgreSQL may behave differently when both operands are \emph{NULL}. For instance, when a JOIN condition involves NULL values, MySQL might not return rows if the comparison between columns involves NULL. Instead, for PostgreSQL, we can use \emph{``IS NOT DISTINCT FROM''} to include the rows where value is NULL. 

{\it (4) Data Types:} MySQL's \emph{DOUBLE} and \emph{DECIMAL} types have precision differences from PostgreSQL' \emph{DOUBLE PRECISION} and \emph{NUMERIC}.


From above failure cases, we can see there are several problems when directly using \llms to conduct dialect translation. 

$\bullet$ \llms may omit some required keywords or translation operations, especially for some lengthy queries.  

$\bullet$ \llms have hallucination problem, like making up functions, cannot tell whether the query can be translated to the target database by its own. 

$\bullet$ \llms may not understand some complex query calculations or expressions, and so they cannot translate into a query with exact same semantic. 

$\bullet$ \llms may fail to match the query syntax of the given database with the syntax of target database, which requires high semantic alignment capability and is crucial for dialect translation.

The translated query in MySQL might look like this:

\begin{verbatim}
SELECT LAST_DAY(CURRENT_DATE) AS result;
\end{verbatim}

In this case, ``DATE\_TRUNC('MONTH', CURRENT\_DATE)'' is replaced with ``CURRENT\_DATE'' since MySQL's ``LAST\_DAY()'' directly returns the last day of the current month. The addition and subtraction of intervals are no longer necessary, as MySQL's ``LAST\_DAY()'' already provides the intended result. Thus, the translated query remains semantically equivalent, ensuring the same behavior on the target database (MySQL) while adhering to its syntax and capabilities.


For instance, the ``NULLS FIRST'' clause is supported in PostgreSQL but may not be correctly translated to other SQL dialects, leading to failures when running queries in those environments. Other functions like ``LPAD'', ``RPAD'', and ``CREATE TABLE a (LIKE b)'' may be misinterpreted across different dialects, leading to failures in translating queries.

\hi{Semantic understanding:} Misinterpretation of keyword presence and command structure. LLMs struggle to interpret the meaning or intent behind certain SQL commands, leading to misclassification of keywords and incorrect translations.

For instance, we may not be able to correctly identify whether keywords are present in a query, or it may omit them entirely, affecting commands such as ``ORDER BY''. These errors cascade into a failure to generate syntactically valid SQL for the target system.

\hi{Subtle syntax differences:} Inability to capture minor but crucial syntax differences. Minor differences between SQL dialects, such as the use of specific functions or slight variations in syntax, can result in translation failures. LLMs might miss these nuances.

For instance, PostgreSQL's ``JSON\_UNQUOTE'' function may not be supported in other SQL variants, which causes issues if LLMs assume uniform support across systems.


\hi{Time zone considerations:} Overlooking the importance of time zone-specific behavior. LLMs may not account for different interpretations of dates and times, especially when dealing with functions that handle time zone-specific data.

For instance, different time functions like ``FROM\_UNIXTIME'' and ``TIMESTAMPADD'' are used. If the model does not account for specific time zone handling in the dialect, this could lead to erroneous time-based queries.

\hi{NULL handling:} Inconsistent behavior with ``NULL'' across different SQL dialects. Handling of ``NULL'' can vary between SQL dialects, and LLMs may not distinguish between these variations accurately, leading to mismatches in query results.

For instance, the system may generate a query where comparisons involving ``NULL'' behave differently across dialects, such as the difference in the interpretation of ``SELECT a IS DISTINCT FROM b'' in some database when ``a'' or ``b'' are ``NULL''.

\hi{Data type translations:} Differences in how data types are handled across SQL dialects may be a source of failure. LLMs might not adapt queries to account for these variations properly.

For instance, translating data types like ``DOUBLE DECIMAL'' incorrectly between systems can lead to query failures if the target dialect does not recognize the data type.

\hi{Model capability limitations:} Incomplete understanding of advanced functions or capabilities. Certain SQL functions or constructs may be entirely missing from LLM-generated queries or incorrectly substituted.

\begin{sloppypar}
For instance, for date functions, PostgreSQL's ``CAST'' or ``DATE\_TRUNC'' may be misinterpreted in MySQL. This could lead to the wrong calculation of date intervals, such as when determining the last day of a month.
\end{sloppypar}


% 过时、解析失败问题、不支持

\llm-based methods can have many problems. 

First, the memorized knowledge (e.g., query syntax) can be out of date.

Real SQLs can be very complex, causing various problems during translation.


Many \llms have been trained with database queries and documents, and can potentially translate different query dialects.

\hi{Missing Translation Knowledge}

How to retrieve and equip LLM with indispensable translation knowledge (e.g., keyword usage description)?


\hi{Hard to Rewrite Lengthy Complex SQL}

%Solution 2: Cross-lingual SQL corpus retriever by contrastive learning.


Short Translation Segment vs. Lengthy Complex SQL. How to identify and simplify the complex real-world queries to be translated?


%Solution 3: Information-guided SQL segmentation + Rule-based SQL normalization.


\subsection{Rule-based Dialect Translation}

We investigate existing query engines that support dialect translation. \zxh{add exp details} We find that these engines all have significant failures. Their translation rules are either incomplete or missing and cannot well cover typical translation cases. Because these rules require expensive manual efforts to maintain existing rules (e.g., supplement query patterns in the condition) and create new rules (e.g., support missing keywords). For instance, \zxh{...}

Therefore, existing translation rule set is incomplete and still needs to be maintained and updated incrementally, and manual-based methods are too costly.

%manual method is too costly to realize sufficiently many rules for translation, which involve typical query keywords, patterns, constraints across different databases. And we need to consider how to discover the translation rules automatically?

%Solution 1: Multi-path LLM-assisted rule generation.


%\zw{Problem Definition.}

% 1. 查询简化（精简的中间语言来方便改写），复杂冗余，提高效率；
\textbf{Observation 1:} 
Only parts of the input queries need to undergo local transformation to adapt to another database system.

% 2. 混合改写，RAG知识匹配算法模型；
\noindent \textbf{Observation 2:}
A hybrid transformation framework that combines the advantages of both techniques can improve performance (i.e., effectiveness and efficiency).

% 3. 规则发现与规则固化。
\noindent \zw{Observation 3:} 
Existing transformation rule set is incomplete and still needs to be maintained and updated incrementally.
\fi

\fi

==> 9_data_sync.tex <==

\iffalse
\section{Unified View for Data Synchronization}
\label{sec:sync}

Due to differing performance and data volume requirements for online and offline feature computations, \oursys typically stores online and offline data in separate physical storage systems. The online storage engine retains only the data necessary for real-time feature computation, applying data expiration policies to manage storage space, while the offline data warehouse preserves the complete dataset for historical analysis. Traditionally, users have to manually maintain synchronization and ensure consistency between online and offline data, which increases maintenance complexity.

To address this problem, \oursys provides an automated data synchronization tool, which consists of two main components: \bfit{(1)~DataCollector} is responsible for capturing data changes in the online engine; \bfit{(2)~SyncTool} receives data from the DataCollectors and writes it to the offline storage engine. SyncTool currently supports writing to the Hadoop Distributed File System (HDFS). Unlike traditional ETL processes that are often batch-oriented and scheduled at fixed intervals, \oursys's automated synchronization tool offers flexible synchronization modes adaptable to data freshness requirements. Synchronization can occur in real-time or at scheduled intervals, depending on the configured mode. 

The tool currently supports three main modes: \emph{(1)~Full Synchronization}, which transfers all existing data at a specific point in time and stops once synchronization is complete; \emph{(2)~Continuous Synchronization with Timestamp Filtering}, which continuously synchronizes data newer than a specified timestamp; and \emph{(3)~Continuous Synchronization of All Data}, which continuously synchronizes all data changes without any filtering.

To optimize synchronization efficiency and resource utilization, \oursys considers the data freshness requirements of different tables. Tables that are less frequently updated can be synchronized at longer intervals, reducing unnecessary data transfer and processing overhead. Conversely, tables that require high data freshness due to frequent updates or critical real-time analytics are synchronized more frequently or in real-time. This adaptive synchronization strategy ensures consistency between online and offline data stores while optimizing system performance.

%Note that in the current version, we only synchronize online tables persistent on the disk engine, which may not be suitable for all use cases, especially those requiring in-memory storage.
\fi

==> embed.tex <==
\section{Cross-Dialect Embedding Model}
\label{sec:embed}

After query processing, another key challenge is matching equivalent syntax in the target database dialect (e.g., functions with identical functionality but different names). However, most existing general-purpose embedding models~\cite{cao2024recent} train on paragraphs from the same documents and do not explicitly consider pairs of cross-dialect specifications. Consequently, they cannot accurately capture the functional similarities of syntax elements across diverse syntax rules and textual descriptions (see Figure~\ref{fig: tsne}).


% are typically trained over \zxh{one dialect's} data (e.g., abstraction and details in one section)}.They 


To address this problem, in this section, we propose \dialectmodel, which generates syntax functionality embedding based on both the syntax tree structure and syntax specification features. Additionally, we employ a retrieval-enhanced contrastive learning approach to effectively synthesize translation samples and train the model with judiciously selected samples (e.g., operation with different functionality but high similarity). %\zw{(e.g., the hard negative samples with different functionality but high similarity).}

% \zxh{cross-lingual} \zw{(i.e., code-level and textual)} s
%positive samples (e.g., functions with the same functionality but different names) and negative samples (e.g., functions that are similar but have different output formats).


% retrieval-enhanced


\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{figures/model_v3.pdf}
  \caption{Cross-Dialect Syntax Embedding Model.}
  % Cross-Lingual Retriever
  \label{fig: model}
  \vspace{-1.5em}
\end{figure}


\subsection{{Model Architecture}}
\label{subsec: model}
%\zxh{Syntactic v.s. semantic}

Given a query syntax \( S^Q \), the goal of \dialectmodel is to encode its functional characteristics by leveraging both syntactic information (i.e., syntax keywords and structures) and semantic information (i.e., textual specifications). This approach ensures that queries with the same functionality, despite having different syntax, keywords, or specifications, will produce similar embeddings and can be effectively matched.

Formally, \dialectmodel is a function $E: \mathcal{S} \rightarrow \mathbb{R}^d$, where $\mathcal{S}$ is the space of all possible query syntax and $d$ is the embedding dimension. The embedding $E(S^Q)$ captures the functionality of the syntax $S^Q$. In this paper, we design the model architecture in a hybrid way to capture different features, which is composed of three main modules:

\bfit{Syntax Structure Encoder.} This module aims to capture the structural features of the query syntax. We utilize a code-based encoder model, such as StarEncoder~\cite{StarEncoder}, which is pretrained on code data (including SQL queries) to extract a structural representation of the query. For the input query $Q$, we first tokenize it into a sequence of tokens $\mathbf{t} = [t_1, t_2, \dots, t_n]$ (e.g., ``\textsf{CONCAT}'', ``\textsf{(}'', ... in Figure~\ref{fig: model}). 
% These tokens represent {keywords, tables, or columns} in SQL. 
We then feed the token sequence into the code-based encoder to obtain the structural embedding $\mathbf{h}_q^{\text{struct}} \in \mathbb{R}^{d_s}$:
\begin{equation}
    \mathbf{h}_q^{\text{struct}} = \text{CodeEncoder}(\mathbf{t})
\end{equation}

The code-based encoder is trained to capture syntactic features of different syntax elements ({e.g., the \textsf{CONCAT()} function in Figure~\ref{fig: model}}), making it suitable for representing syntax structures.

%with the encoder built upon an open-source code-based encoders (e.g., Starencoder~\cite{StarEncoder} \zw{}).

\bfit{Syntax Specification Encoder.} Since different dialect specifications show diverse writing styles (e.g., {the \textsf{CONCAT()} function in MySQL$\footnote{\blue{\url{https://dev.mysql.com/doc/refman/8.4/en/string-functions.html\#function\_concat}}}$ is detailed with illustrative examples, while the one in PostgreSQL$\footnote{\blue{\url{https://www.postgresql.org/docs/14/functions-string.html}}}$ is succinct as one row)}, this module employs multiple natural languages (NL)-based encoders to capture multi-dimensional features of specifications and acquire a weighted representation of the specification in a mixture-of-experts (MoE) style.
% MySQL specifications provide detailed examples, while the ones in PostgreSQL are more succinct

\begin{sloppypar}
Let $\mathbf{d}$ denote the textual specification associated with the query syntax $S$. We employ a set of $K$ NL-based encoders $\{\text{NLEncoder}_k\}_{k=1}^K$, each capturing different aspects of the specification. For instance, some encoders can extract information from long passages, while others are skilled at representing short paragraphs~\cite{MTEB}.
% while others might specialize in understanding technical jargon. 
Each encoders generates an embedding vector, i.e., $\mathbf{h}_{q,k}^{\text{desc}} = \text{NLEncoder}_k(\mathbf{d}) (k = 1, \dots, K$).
\end{sloppypar}

We then aggregate these embeddings using a gating mechanism to obtain the final specification embedding $\mathbf{h}_q^{\text{desc}}$:
\begin{equation}
    \mathbf{h}_q^{\text{desc}} = \sum_{k=1}^K \alpha_k \mathbf{h}_{q,k}^{\text{desc}}
\end{equation}
where $\alpha_k$ are the gating weights determined by a gate function:
\begin{equation}
    \alpha_k = \frac{\exp(g_k(\mathbf{d}))}{\sum_{j=1}^K \exp(g_j(\mathbf{d}))}
\end{equation}
where $g_k(\mathbf{d})$ is the output of the gating network for the $k$-th encoders, allowing the model to dynamically assign weights based on the input specification. For instance, a higher weight for encoder specialized in understanding and encoding the detailed illustrations about the \textsf{CONCAT} function in MySQL.

% For instance, suppose we have two natural language (NL) model as encoders, i.e., \textit{Encoders 1} (specialized in processing long, detailed specifications \zxh{(add ref)}) and  \textit{Encoders 2} (specialized in understanding concise, technical definitions \zxh{(add ref)}). Given a long paragraph explaining the query syntax, the gate function may assign a higher weight to \textit{encoders 1}, emphasizing its contribution to the final embedding.

%Since different dialect documents showcase diverse writing styles (e.g.,  MySQL specifications provide detailed examples, while PostgreSQL has much fewer examples), this module employs multiple NL-based encoderss (e.g., the ones in the MTEB leaderboard\footnote{\url{https://huggingface.co/spaces/mteb/leaderboard}}) to acquire a weighted representation of specification in an MoE style. These encoderss have their own advantages, e.g., some encoderss are good at extracting from long-term paragraphs, and others ....  Specifically, each NL-based encoders captures the features of specifications in one dimension and finally aggregates the generated through a gate function.


\bfit{Structure-Specification Aggregator.} Given the syntax structure embedding $\mathbf{h}_Q^{\text{struct}}$ and the specification embedding $\mathbf{h}_Q^{\text{spec}}$, this module combines the two features using a multi-head cross-attention. It ensures that the model focuses on the most relevant parts of the specification in relation to the syntax structure, i.e.,
\begin{equation}
    \mathbf{E}(q) = \text{CrossAttention}(\mathbf{h}_q^{\text{struct}}, \mathbf{h}_q^{\text{desc}})
\end{equation}
\begin{sloppypar}

\noindent where $\text{CrossAttention}$ $\mathbf{E}(q) = {Concat}({head}_1, \dots, {head}_h) \mathbf{W}^O$, each head ${head}_i = \text{Attention}(\mathbf{h}_q^{{struct}} \mathbf{W}_i^Q, \mathbf{h}_q^{{desc}} \mathbf{W}_i^K, \mathbf{h}_q^{{desc}} \mathbf{W}_i^V)$. The attention function is defined as  %\zxh{tbd: add example}
\end{sloppypar}
\begin{equation}
    \text{Attention}(Q, K, V) = \text{softmax}\left(\frac{Q K^\top}{\sqrt{d_k}}\right) V
\end{equation}
where $\mathbf{W}_i^Q$, $\mathbf{W}_i^K$, $\mathbf{W}_i^V$, and $\mathbf{W}^O$ are projection matrices, and $d_k$ is the dimension of the keys.

In this way, we can align and integrate information from both embeddings, effectively filtering out irrelevant parts of the specification and focusing on syntax-relevant content. Continuing from previous examples, suppose the specification includes query syntax descriptions and usage hints. The cross-attention mechanism will assign higher attention weights to relevant parts (e.g., {the example SQL query and its illustrations about \textsf{CONCAT}}), integrating them with the structural embedding to produce the final embedding $\mathbf{E}(q)$.

In summary, the advantages are three-fold. {\it (1) Robustness to Syntax Variations:} The model {incorporates} the functional characteristics of different database dialects, making it resilient to variations in query syntax elements and rules. {\it (2) Adaptability to Diverse Specifications:} Using an MoE-style Syntax Specification Encoder, we can process specifications of varying lengths and styles by assigning appropriate weights to different NL-based encoders.  {\it (3) Effective Feature Integration:} The multi-head cross-attention integrates only the most relevant descriptive features with syntax elements, improving the ultimate functionality embedding quality.

%Given the syntax structure and specification embedding features derived from the aforementioned modules, this module combines the two features based on a multi-head cross-attention mechanism. Specifically, the textual features are aggregated based on their attention scores over the code-specific features (e.g., remove the redundant sentences and only retain the code-relevant parts in the specifications).

%built upon \zxh{an open-source code-based encoders} is utilized to capture code-specific features for the input SQL segment (i.e., keyword); 

%leverages diverse \zxh{NL-based encoderss} to embed the input functionality specifications in different aspects; 


%incorporates both the code and textual features via the cross attention mechanism \zxh{to align the code and textual embedding (e.g., code of different keywords can have the same semantic)}.


\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{figures/training_v4.pdf}
  \caption{Illustration of Retrieval-Enhanced Contrastive Learning (\emph{Green:} Positive Sample; \emph{Red:} Negative Sample).}
  \label{fig: training}
    \vspace{-1.5em}
\end{figure}

\subsection{Retrieval-Enhanced Contrastive Learning}
\label{subsec:train}

Next, we explain how to effectively train \dialectmodel with limited samples. Training this model requires a substantial number of positive and negative samples to distinguish between functionally equivalent syntax elements and those that are not~\cite{DBLP:journals/entropy/Albelwi22}. Positive samples are pairs of syntax elements with the same functionality, while negative samples are pairs that differ functionally.  

However, despite the availability of numerous queries from different dialects, obtaining equivalent pairs based on their annotated specifications is challenging (e.g., there are 735 candidate PostgreSQL specifications and 532 MySQL specifications). To address this issue, as illustrated in Figure~\ref{fig: training}, we first introduce methods to automatically generate these samples as initial training data. We then present a novel retrieval-enhanced contrastive learning paradigm to train the model using the generated samples.

\subsection*{5.2.1 Training Sample Generation} 

For each database system, we collect query syntax trees and specifications from official syntax documentation (see Section~\ref{subsec:spec-gen}). We represent each type of query syntax tree as a pair of syntax elements and specifications, i.e., \( s_i = \langle Q^s_i, \mathbf{d}^s_i \rangle \), where \( Q^s_i \) denotes the query keywords or structure, and \( \mathbf{d}^s_i \) represents the textual specification. For each syntax element (an anchor element), we generate positive and negative samples based on the following strategies:

\hi{Positive Sample Generation}. As shown in Figure~\ref{fig: training}, we synthesize positive samples using the following methods.

\bfit{M1:} {\it Self-Augmented Specifications.} For a syntax $s_i$, we perform self-augmentation on its specification $\mathbf{d}^s_i$ by rephrasing sentences, replacing words with synonyms, and permuting sentence order~\cite{nlpaug}. Each augmented specification $\mathbf{d}^s_i'$ forms a new syntax pair $\langle Q^s_i, \mathbf{d}^s_i' \rangle$. The original syntax pair and each augmented pair form positive sample pairs, reinforcing the model's robust understanding of varying expressions of the same functionality~\cite{AdvTraining, TRAP}.

\bfit{M2:} {\it Cross-Database Specifications.} For a syntax $s_i$, we search for syntax \( s_j \) in other databases that has the same {keywords of identical functionality} but different specifications. For example, built-in functions in both MySQL and PostgreSQL may have different specification styles discussed in Section~\ref{subsec: model}. Pairs \( (s_i, s_j) \) form positive samples, helping the model recognize equivalent functionalities across different database dialects.
 
\bfit{M3:} {\it Tool-Based Translations.} For a syntax $s_i$, we utilize existing dialect translation tools (e.g., SQLGlot) to translate the query \( Q^s_i \) of syntax \( s_i \) into other database dialects, producing new queries \( Q^s_k \). Each translated query combined with its corresponding specification forms a new syntax \( s_k = \langle Q^s_k, \mathbf{d}^s_k \rangle \). The pairs \( (s_i, s_k) \) serve as positive samples.

%we search for the syntax $s_j$ which the specifications with different keywords but identical functionality based on the translations of existing translators (e.g., xxx in MySQL and xxx in PostgreSQL).

\hi{Negative Sample Generation}. After generating positive samples, we cluster syntax elements based on their functional equivalence, i.e., syntax elements that are positive samples with each other are grouped into the same cluster. To construct negative samples, we consider pairs of syntax elements from different clusters whose size is large than one, which are expected to be functionally different.

%selection of specifications with different SQL keywords.


\subsection*{5.2.2 Contrastive Model Training} 

Given the generated samples, contrastive model training aims to (1) reduce the distances between embeddings of positive samples (pulling them closer), and (2) increase the distances between embeddings of negative samples (pushing them apart). For any syntax \( s_i \) as an anchor sample, we obtain its positive samples \( \mathcal{P}(i) \) and negative samples \( \mathcal{N}(i) \). The \dialectmodel\ encodes each syntax \( s \) into an embedding vector \( \mathbf{h}_s = f_\theta(s) \).

\hi{Hard-Negative Sample Selection.} Within the set \( \mathcal{N}(i) \), many negative samples are either (1) already well-distinguished from \( s_i \)'s embedding (i.e., with low cosine similarity), or (2) introduce significant noise due to their dissimilarity or irrelevance. To alleviate the efforts spent on such ineffective samples, we introduce \textbf{hard negative samples}, i.e., samples that (1) have different functionality from \( s_i \) but (2) possess embeddings similar to that of \( s_i \).
{For example, the specification of function A is redundantly referred to by the specification of function B, which leads to the matching for function A mistakenly occurring for function B.}
% For example, the opposite operations \textsf{GRANT} and \textsf{REVOKE} separately grant and remove user privileges but may have similar embeddings due to shared syntax \zxh{replace the example}.
To derive the set of hard negative samples \( \mathcal{N}'(i) \), we first select negative samples whose embeddings are more similar to \( s_i \) than those of any positive samples (i.e., they are ranked higher in similarity). 
% If the number of these samples is smaller than a predefined threshold (\zxh{how?}), we randomly select additional negative samples from the remaining \( \mathcal{N}(i) \) to meet the required number.

\hi{Loss Function Design.} Using the samples in \( \mathcal{P}(i) \) and \( \mathcal{N}'(i) \), we design the contrastive loss function for \( s_i \) as:

\[
\mathcal{L}_i = -\frac{1}{|\mathcal{P}(i)|} \sum_{s_p \in \mathcal{P}(i)} \log \left( \frac{ \exp(z_{ip}) }{ \exp(z_{ip}) + \sum_{s_n \in \mathcal{N}'(i)} \exp(z_{in}) } \right)
\]
where $z_{ij}$ denotes the scaled cosine similarity between embeddings \( \mathbf{h}_{s_i} \) and \( \mathbf{h}_{s_j} \), i.e., $z_{ij} = {\text{sim}(\mathbf{h}_{s_i}, \mathbf{h}_{s_j})}/{\tau}$. \( \tau \) is a temperature hyper-parameter controlling the {concentration level of the distribution}. \( z_{ip}\) is the scaled similarity of $s_i$ with a positive sample, and \( z_{in}\) is the scaled similarity of $s_i$ with a hard negative sample.

This loss function encourages the model to maximize the similarity between the anchor sample and its positive samples while minimizing the similarity with hard negative samples.

\iffalse
\begin{equation}
\footnotesize
\mathcal{L}_i = -\frac{1}{|\mathcal{P}(i)|} \sum_{s_p \in \mathcal{P}(i)} \log \frac{\exp\left( \frac{\text{sim}(\mathbf{h}_{s_i}, \mathbf{h}_{s_p})}{\tau} \right)}{\exp\left( \frac{\text{sim}(\mathbf{h}_{s_i}, \mathbf{h}_{s_p})}{\tau} \right) + \sum_{s_n \in \mathcal{N}'(i)} \exp\left( \frac{\text{sim}(\mathbf{h}_{s_i}, \mathbf{h}_{s_n})}{\tau} \right)},
\end{equation}
where \( s_n \) denotes a hard negative sample in $\mathcal{N}'(i)$, \( \text{sim}(\mathbf{h}_{s_i}, \mathbf{h}_{s_j}) = \frac{\mathbf{h}_{s_i}^\top \mathbf{h}_{s_j}}{\|\mathbf{h}_{s_i}\| \|\mathbf{h}_{s_j}\|} \) is the cosine similarity between embeddings, \( \tau \) is a temperature hyper-parameter controlling the concentration level of the distribution,  \( |\mathcal{P}(i)| \) is the number of positive samples for \( s_i \).

This contrastive loss function encourages the model to maximize the similarity between \( s_i \) and its positive samples while minimizing the similarity with negative samples. \zxh{add dialect relevant insights}

%Given a data sample (i.e., an anchor), the rationale of contrastive learning is to minimize the distance over the similar samples (i.e., positive samples) and, in contrast, maximize the distance over the different samples (i.e., negative samples).

\zw{rephrase with the concept of retrieval}
\fi

==> query.tex <==
%First, to remove \zw{unusual translation-irrelevant} parts (e.g., functions, reserved keywords), \processor normalizes the query by replacing these parts with expressions composed of common operators using keyword matching.  Second, to segment the query, \processor constructs a hierarchical tree based on BNF syntax and splits the query according to the BNF tree. To reduce the side-effect \zw{(statistics)} of redundant query parts, \processor simplifies each operation by only reserving the keywords used in the matched syntax and abstracting the rest of the parts.

\section{Functionality-based Query Processing}
\label{sec: processor}

In this section, we introduce how to properly process the input queries with various structures and operations, including syntax functionality annotation, tree-based query segmentation, and rule-based query simplification.

\subsection{Syntax Functionality Annotation} 
\label{subsec:spec-gen}

Given a database dialect, we extract the syntax elements from its query parser files (e.g., the gram.y file in PostgreSQL). For each syntax element \( S \), we require (1) the syntax tree in Backus-Naur Form (BNF) of $S$ for exact syntax matching and (2) the specification of $S$'s functionality for future translation (see Section~\ref{sec: translate}). 

\emph{(1) Syntax Tree Generation:} Different database parsers follow diverse rules, making their parsed syntax trees difficult to compare. To achieve syntax matching across databases, we generate syntax trees in a unified BNF format. We maintain and use a series of BNF definitions~\cite{BNF} to standardize the syntax representation of queries. And, for every database, we derive the syntax trees of syntax elements in the database, where the leaf nodes represent BNF terminal symbols (e.g., literals), and the internal nodes represent non-terminal symbols (e.g., SQL clauses, functions).

\emph{(2) Syntax Specification Annotation:} For the BNF-based syntax tree of $S$, we annotate functionality specifications by exact syntax element matching. We start by comparing the syntax tree nodes of $S$ with those from syntax elements in sources like official documents (e.g., PostgreSQL, MySQL, and Oracle separately offer 245, 466, and 490 pages). using a depth-first traversal. Next, we annotate the matched subtrees (query operations) of $S$ with their corresponding syntax trees and specifications, including $(i)$ functionality, $(ii)$ usage constraints, $(iii)$ arguments and default values, and $(iv)$ usage examples, all of which are vital for syntax matching and translation. For instance, since the keyword \textsf{AS} appears in various rules (e.g., in the \textsf{CAST} function or as a column and table alias), we differentiate specifications for \textsf{AS} based on the relevant syntax trees.

%we annotate the syntax elements and specification of  from both  \zxh{check the example}.

% \emph{(1) Syntax Tree Generation:} Different database parsers can have diversified rules and their parsed syntax tress can hardly be compared. Thus, to support syntax matching across databases, we generate syntax trees in unified BNF formats. To this end, We maintain and utilize a series of BNF definitions to get the standard syntax expression for each syntax element in the query. Specifically, we derive the syntax trees for syntax elements of queries from different databases, where the leaf nodes denote BNF terminal symbols (e.g., keywords, literals) and internal nodes denote non-terminal symbols (e.g., SQL clauses, function calls).

% For databases like MySQL, we can reuse existing BNF pasers (e.g., \zxh{add}). Instead, for a database without BNF parser, we first locate the database's parser files (e.g., \zxh{xxx file in DuckDB}). Then, we transform the syntax rules in the parser into BNF notation with non-terminals and terminals. 

% For the BNF-based syntax tree of $S$, we annotate the functionality specifications (e.g., from database documents) by matching the above syntax elements (i.e., exact comparison of the syntax tree nodes in a bottom-up manner), including

% syntax matching
% 基于语法构架SQL语法树，然后每个匹配，为树上结点带上offline preparation阶段处理的description等其他信息
\subsection{Tree-based Query Segmentation} 

Next, we discuss how to segment queries based on the syntax trees of different functionalities. There are generally two strategies: 

%\zw{can be shorter}

\emph{(1) Lexical-Based Segmentation} uses regular expressions to split an SQL query based on specific keywords or patterns. Typical SQL keywords such as \textsf{SELECT} serve as markers to divide the query into smaller parts. However, it treats the query as a flat sequence of tokens, ignoring the underlying syntax and the hierarchical relationships in the query (e.g., subqueries within \textsf{SELECT} and \textsf{WHERE} clauses depend hierarchically on the outer query). 

\emph{(2) Tree-Based Segmentation} conducts an exact matching of sub-trees in the query's syntax tree for capturing the query structures. 

Lexical-based segmentation struggles with complex queries (e.g., with nested subqueries). For these queries, the operations derived by lexical-based segmentation may incorrectly span across multiple clauses. Thus, we adopt the tree-based strategy. Similar to {\it syntax specification annotation}, we traverse syntax tree $T^Q$ in a {depth-first order} to match the predefined syntax elements. We denote the exact matching function as \( M(t) \), which returns \textsf{TRUE} if the substree \( t \) matches that of an element in the dialect syntax \( S \), and \textsf{FALSE} otherwise. If a match is found, we extract the subtree \( t \) rooted at node \( \mathcal{N}_k \). This subtree corresponds to the operation that begins at \( \mathcal{N}_k \), such as the \textsf{SELECT} clause. The tokens contained in \( t \) are then converted back into SQL query, i.e., \( q = \text{Unparse}(t) \). In this way, we ensure that all tokens within the subtree \( t \) belong to the same operation (e.g., all tokens in the \textsf{SELECT} clause are kept together).

After syntax matching, we aggregate these identified operations, i.e., \( Q = \{q_{j} \mid M(t) = \text{True}\} \). Each operation \( q_{j} \) forms a valid SQL expression annotated with functionality specifications (obtained in Section~\ref{subsec:spec-gen}), which can then be used in translation.

%We format the input SQL (e.g., upper all the SQL keywords) and build a hierarchical tree with the BNF grammar, where the leaf nodes correspond to the SQL tokens and the non-leaf nodes correspond to the SQL components (e.g., the SQL clauses)$\footnote{Note that we implement and maintain the tree builder based on the grammar for different database dialects.}$. Then, we traverse the tree in \zw{a top-down manner} by matching the SQL keywords which are also parsed into trees.

%Once a successful matching occurs, \processor operations the queries by extracting the subtree starting from the non-leaf node and make sure the extracted SQL tokens are all within the same clause.

% normalization and abstraction

\vspace{-1.25em}
\subsection{Rule-based Query Simplification}
\label{subsec:simplify}

{Based on the observation in Section~\ref{sec:mot}}, when translating SQL queries between different dialects, it is essential to simplify operations by (1) replacing customized functions (e.g., \textsf{LAST\_DAY()} in MySQL) with equivalent common ones and (2) focusing on syntax elements that are crucial for accurate translation. Therefore, we employ predefined rules to further process operations segmented from the query $Q$, retaining only the translation-relevant components. 

The core principle of this simplification is to ensure that within the syntax subtree of an operation, no nodes contain customized functions, and any non-leaf nodes that do not affect translation are replaced with predefined terms or query templates. To this end, we provide simplification rules in the three main scenarios:

%\noindent$\bullet$ \emph{Case 1: Simplifying Customized Functions.} Database systems often implement a wide range of customized functions for ease of use {(e.g., the \textsf{LAST\_DAY} function involves the same calculation based on \textsf{DATE\_TRUNC()} function in PostgreSQL)}.   However, these functions are often unsupported or behave inconsistently across different databases. To address this, we maintain mappings {(from SQLGlot or identified by human expertise)} of customized functions to equivalent SQL expressions of common functions (if they exist) for query normalization. For instance, with the rule ``\textsf{str ILIKE pattern::=LOWER(str) LIKE LOWER(pattern)}'' \zw{SYN},  we normalize PostgreSQL’s case-insensitive \textsf{ILIKE} function into the standard SQL expression using \textsf{LIKE} with lowercase transformations.

\noindent$\bullet$ \emph{Case 1: Simplifying Customized Functions.} Database systems often implement a variety of customized functions to enhance usability (e.g., the \textsf{LAST\_DAY} function in PostgreSQL). However, these functions are often unsupported or exhibit inconsistent behavior in other database systems. To tackle this issue, we maintain mappings (sourced from SQLGlot and human expertise) of customized functions to equivalent expressions using common functions (if available) for query normalization. For example, with the rule ``\textsf{str ILIKE pattern::=LOWER(str) LIKE LOWER(pattern)}'', we normalize PostgreSQL’s case-insensitive \textsf{ILIKE} function into the standard SQL expression by applying \textsf{LIKE} with lowercase transformations.


% , which performs the same calculation based on the \textsf{DATE\_TRUNC()} function


%\zw{Besides, there might exist redundant customized functions that can be implemented via the combination of other functions.}
% For example, PostgreSQL’s \textsf{TO\_TIMESTAMP()} converts a double precision value into a timestamp, while MySQL’s \textsf{FROM\_UNIXTIME()} formats a UNIX timestamp. 

% \textsf{SPLIT\_PART(str, delimiter, 1)::= SUBSTR(str, 1, POSITION(delimiter IN str) - 1)}

\begin{sloppypar}
\noindent$\bullet$ \emph{Case 2: Abstracting Irrelevant Expressions.} Some functions or expressions nested within an operation $q_i$ are generally not used when translating $q_i$. For instance, consider the operation ``\textsf{CAST(CONCAT(`DR\texttt{.}\'', `', name) AS TEXT)}'', which is matched by the \textsf{CAST} syntax. The inner \textsf{CONCAT} function does not affect the translation of the \textsf{CAST} operation and can be abstracted away. As a result, the expression is simplified to \textsf{CAST(column\_expr AS TEXT)}, where \textsf{column\_expr} represents a non-terminal symbol.
\end{sloppypar}

\noindent$\bullet$ \emph{Case 3: Abstracting Irrelevant Query Clauses.} Certain query clauses may not be relevant to the primary function or behavior of a specific syntax and can be masked. For instance, in the MySQL query ``\textsf{SELECT * FROM child WHERE age >= 10 LIMIT 2 OFFSET 10}'', which is matched by the \textsf{LIMIT} syntax, the \textsf{SELECT} clause and \textsf{WHERE} condition are not relevant to the translation of the \textsf{LIMIT} clause. Thus, these parts can be masked, retaining only the \textsf{LIMIT} portion, i.e., \textsf{select\_stmt LIMIT 2 OFFSET 10}.


%Therefore, we propose to transform a customized function into equivalent SQL expression composed of common operations. First, we generate an Abstract Syntax Tree (AST) from the source code of the function, breaking it down into meaningful components like loops, conditionals. Second, we traverse the AST to identify key operations such as function calls (e.g., interval\_subtract\_timestamps in the \textsf{AGE} function), arithmetic operations, and logical comparisons. Third, we map these code-level operations to their SQL equivalents by creating a mapping between them (e.g., mapping interval\_subtract\_timestamps to \textsf{TIMESTAMPDIFF} in SQL), replacing the original operations in the AST and adjusting the structure to align with SQL syntax. Fourth, we generate the SQL query string by traversing the transformed AST, assembling operations and operands in the correct order to form a syntactically valid SQL expression (e.g., {\textsf{\dots TIMESTAMPDIFF(YEAR, \dots, \dots) AS AGE \dots}}). 

%Finally, we perform functional validation by creating test cases with inputs (e.g., two dates for TIMESTAMPDIFF) and expected outputs, running both the function and the new SQL expression to compare results and ensure the transformation's correctness. In this way, we maintain such pairs of customized function and SQL expression for query normalization.


% Moreover, we support advanced abstractions that can leverage incompatibility warnings related to function arguments and operands. For instance, \zxh{given a warning such as ``{\it operator does not exist: text + text}'', the operation ``\textsf{`2024-10' + salary}'' can be abstracted to ``\textsf{str\_column + salary}''.} This type of abstraction is more challenging to generalize into standard rules and often requires careful, case-by-case analysis.

\iffalse
\begin{example}
Consider the example query in Figure~\ref{fig:overview}. First, the syntax tree includes \textsf{SELECT}, \textsf{FROM}, and \textsf{WHERE} clauses as the main branches. Then, during tree traversal and matching, we start at the root of the tree and match the \textsf{SELECT} clause, extracting the entire \textsf{SELECT} clause, which includes the complex expression \textsf{CAST(concat('a', 'b', name) AS TEXT) AS Result}; next, it separately traverses the \textsf{FROM} and \textsf{WHERE} clauses. In this way, we split the origin query into three operations: (1) \textsf{SELECT CAST(concat('a', 'b', name) AS TEXT) AS Result}, (2) \textsf{FROM people}, and (3) \textsf{WHERE EXTRACT(YEAR FROM AGE(CURRENT\_DATE, birthday)) < 70}. 
\end{example}
\fi

% This abstraction allows us to generalize the translation of the `CAST` function without concerning ourselves with the specifics of the inner expression.
% consider the operation \textsf{CAST(CONCAT(`a', `b', name) AS TEXT)}, which matches the \textsf{CAST} syntax. The inner \textsf{CONCAT} function does not impact the dialect translation of the  \textsf{CAST} operation and can therefore be abstracted away. We simplify the expression to \textsf{CAST(column\_expr AS TEXT)}, where column\_expr is a non-terminal symbol representing any column expression. This abstraction allows us to generalize the translation of the \textsf{CAST} function without concerning ourselves with the specifics of query expressions.



%For instance, for the MySQL query \textsf{SELECT * FROM child WHERE child.age >= 10 LIMIT 2 OFFSET 10} matched by the \textsf{LIMIT} syntax, we can directly mask the \textsf{SELECT} clause and only reserve the \textsf{LIMIT} part, i.e., \textsf{select\_stmt LIMIT 2 OFFSET 10}.

% advanced abstraction techniques can involve masking query components


% \zw{1. abstract the table and column names;
% 2. synthesize simple query (SELECT *) to replace the original}




\iffalse
\hi{Code AST Generation.} With the source code of a customized function, we convert the source code into an Abstract Syntax Tree (AST), a hierarchical structure that represents the syntactic structure of the code. For C-based code, using a compatible parser like a C parser, the AST helps break the function into meaningful components (e.g., loops, conditionals, function calls). For instance, parsing the \textsf{AGE} function from PostgreSQL will generate an AST that shows its internal logic \zxh{add}.

\hi{Code Operation Identification.} By traversing the AST of the function, we systematically locate function calls, arithmetic operations, and logical comparisons. For instance, in the \textsf{AGE} function, we can automatically find operations like {\it interval\_subtract\_timestamps}, which need to be clearly identified and recorded. The AST helps by visually organizing these operations in the order they are executed.


\begin{sloppypar}
\hi{SQL Operation Mapping.} With the identified operations, next we translate language-specific operations into SQL equivalents. To do this, we create a mapping between the code-level operations and SQL operations. For instance, if the original C code contains {\it interval\_subtract\_timestamps}, the SQL equivalent might be \textsf{TIMESTAMPDIFF}. Similarly, arithmetic operations in C are directly mapped to their SQL counterparts. Here we use a dictionary or table to maintain this mapping, ensuring all necessary operations have SQL equivalents. \zxh{check} After mapping the operations, we replace the code-specific operations with SQL equivalents and adjust the structure of the tree by following the SQL syntax. 
\end{sloppypar}

%For example, the AST node representing {\it interval_subtract_timestamps} would be transformed into a {\it TIMESTAMPDIFF} SQL function call. The hierarchical structure of the AST must be preserved, but its nodes must now align with SQL’s syntax rules.

\hi{SQL Expression Generation.}  With the transformed AST, we traverse the tree and construct the SQL query string. To ensure all operations and operands are assembled in the correct order to create a syntactically valid SQL expression, starting from the root of the AST, we generate the SQL by combining operators and operands as they appear in the tree. For instance, after transforming the AST of the \textsf{AGE} function, we generate a SQL query like ``\textsf{$\cdots$ TIMESTAMPDIFF(YEAR, `birth\_date', CURRENT\_DATE) AS AGE $\cdots$}''. \zxh{check}


\hi{Functional Validation.} Finally, we automatically create some test cases with known inputs and expected outputs \zxh{check}, running both the original customized function and the new SQL expression, and comparing the results. For example, using various timestamp inputs, you would confirm that both the AGE function and its SQL equivalent return the same age calculations. This step ensures the functional correctness of the transformation.

We can memorize the pair of customized function and its SQL expression for future reuse. That is, once we have translated a customized function into its equivalent SQL expression, we store this mapping in a lookup table. This allows for quick reference and reuse in subsequent query normalization.
\fi


 %As shown in Figure~\ref{} \zw{(same figure to be added)}, the query operations by lexical-based segmentation are originated from different clauses. However, lexical-based segmentation treats the query as a flat string and ignores the underlying syntax and hierarchical structure, which cannot extract the valid query operations accurately. 

%, which leverages the syntactic structure of the query. By analyzing the AST, \processor can accurately identify query components and preserve the logical relationships between them. This method ensures that the operations are valid, self-contained, and reflective of the query's intended meaning, even when dealing with complex SQL structures.










\iffalse
\llm is prone to produce hallucination when given lengthy input. Besides, it might be lost in the input contexts and fail to grasp the core information for dialect translation~\cite{}.
Our experimental studies shown that \llms fail to handle the complex SQL queries with diverse issues (randomly discard some SQL tokens demonstrated in Section~\ref{}). Therefore, we first manage to simplify the input queries and enhance \llm to generate accurate and reliable dialect translation for small query operations.

Our key observation is that for most of the queries, only parts of them are required when conducting translation.
For example, only the xxxx are required for translation as shown in Figure~\ref{} \zw{(a concrete example to be added)}.
Based on this observation, we propose to 
\fi




\iffalse
(1) Knowledge preparation

重新组织文档构建索引（关键词序列）

(2) Identify and segment the queries to be transformed;

transform complex function into atomic operators (last\_day --> expression)



% udf function; storage process (do not consider)

% translation: functions originally supported by all the database proceducts, but only syntax is different; 

% 对象类型

% 数据类型；关键词；内置函数（关键词）；语法


(3) Simplify the expression of the segmented queries.

\fi

==> translate.tex <==

\iffalse
We first identify problematic query operations based on parsing errors encountered during query processing. The process involves the following steps:

{\it (1) Parsing Error Detection:} The input query (\(Q\)) is parsed, and any syntax or structure that causes a parsing error is flagged.

{\it (2) operation Selection:} The operations causing these errors are isolated as smaller translation units. For example, in the figure, operations like FUNC\_EXPR and CAST are identified for further processing due to their parsing issues.

{\it (3) operation Extension:} If the selected operation, once translated, causes further errors in the revised query (\(Q'\)), the method dynamically extends the operation to cover the newly problematic areas, allowing for a more comprehensive translation.
\fi

% ($Q$, $source\_dialect$, $target\_dialect$)
\begin{figure}[!t]%\vspace{-1em}
\removelatexerror
\begin{algorithm}[H]
\label{alg:translate}
\caption{LocalToGlobalDialectTranslation}
\KwIn{Origin Query $Q$; $source\_dialect$; $target\_dialect$}

Initialize the translated query $Q'$ as $Q$\;
\Repeat{no incompatibility warnings \textbf{or} arriving maximal trials}{
    $incompatible\_ops$ = \textbf{DetectIncompatibility}($Q'$, $target\_dialect$)\;
    \ForEach{$op$ in $incompatible\_ops$}{
        \Repeat{$translated\_op$ is not None \textbf{or} cannot extend $op$}{
            $translated\_op$ = \textbf{Translate}($op$, $target\_dialect$)\;
            % \If{$translated\_op$ is Error}{
            %     \textbf{break} \tcp*{Unsupported Operation}
            % }
            \If{$translated\_op$ is not None}{
                Replace $op$ with $translated\_op$ in $Q'$\;
            } \Else{
                Extend $op$ to include more operations in $Q'$\;
            }
        }
    }
}

\If{\textbf{ValidateQuery}($Q'$, $Q$, $target\_dialect$)}{
    \Return $Q'$ \tcp*{Translation successful}
}
{
    \Return {Error} \tcp*{Translation failed}
}
\end{algorithm}

\begin{function}[H]
\label{func:detect}
\caption{DetectIncompatibility($Q$, $target\_dialect$)}
\KwIn{Query $Q$; $target\_dialect$}
Generate the syntax tree of $Q$ in $target\_dialect$ BNF definitions\;
Collect incompatibility warnings\;
{Identify the operations causing each warning}\;
\Return list of operations causing incompatibility warnings\;
\end{function}

\begin{function}[H]
\label{func:translateop}
\caption{Translate($op$, $target\_dialect$)}
\KwIn{Operation to translate $op$; $target\_dialect$}

% \If{$op$ can be translated by a rule engine}{
%     \Return translated $op$ by the rule engine\;
% }

Match $op$ with relevant syntax in $target\_dialect$\;

% \If{syntax match is not found}{
%     \Return Error \tcp*{Unsupported Operation}
% }

{Use LLM to translate $op$ within maximal trials\;}


\If{$translated\_op$ is valid \textbf{and} {equivalent to $op$}}{
        \Return $translated\_op$
}
\Return None \tcp*{Translation failed}
\end{function}

\vspace{-2em}
\end{figure}


\section{Local-To-Global Dialect Translation}
\label{sec: translate}

% Rather than merely relying on translation tools or \llms, 
% To deal with the correlations among different query operations, i
To translate queries with various syntax elements, in this section we propose a Local-To-Global algorithm that conducts focused translations over potentially incompatible operations (see Algorithm~\ref{alg:translate}).
%It translates potentially incompatible query operations (Section~\ref{sec: processor}) using \llm informed by the specifications via model-based syntax matching (Section~\ref{sec:embed}), {gradually extends the query operations and} refines the translations to ensure both syntactic correctness and functional equivalence (see Algorithm~\ref{alg:translate}).

% Translating the query operations between different dialects poses significant challenges due to variations in {\it syntax, supported functions, and \zxh{database-specific features}}. To this end, we present

\hi{Validation-Guided Operation Selection.} 
Since not all the query operations require translation (discussed in Section~\ref{sec:mot}), we identify query operations that are (1) incompatible with the target database dialect or (2) cannot be correctly translated with its local syntax tree and specification. 
% This selection is guided by incompatibility warnings encountered \zw{during the generation of the syntax tree with the target dialect BNF definitions}.
% during initial query processing.

\textit{(1) {Incompatibility Warning} Detection.} 
We try to generate the syntax tree for the input query \(Q\) based on the {BNF} definitions in the target dialect. 
Any syntax element that raises incompatibility warnings during the tree generation is flagged to be translated. 
For instance, consider the PostgreSQL SQL in Figure~\ref{fig:overview}, the ``\textsf{CAST(CONCAT('a', 'b') AS TEXT)}'' casts the result of \textsf{CONCAT} function into the \textsf{TEXT} type. 
However, the \textsf{TEXT} type is not allowed in the \textsf{CAST} function of MySQL.
Thus, the \textsf{CAST} function raises an error and is flagged.
% parsed by a dialect in MySQL, it warns ``{\it syntax error near `::date'}'' since it does not support this syntax.

\iffalse
\textit{(1) Incompatibility Error \zw{syn} Detection.} We parse the input query \(Q\) using the target database's SQL parser \zw{BNF}. Any syntax elements that cause incompatibility warnings are flagged to be translated. For instance, consider the PostgreSQL query ``\textsf{SELECT * FROM employees WHERE hire\_date::date = `2023-01-01'}'', the ``::date'' casting operator is specific to PostgreSQL. When parsed by a dialect in MySQL, it warns ``{\it syntax error near `::date'}'' since it does not support this syntax.
\fi

\textit{(2) Operation Selection.} The operations raising the incompatibility warnings are isolated as smaller translation units. Continuing the above example, the problematic query operation is the \textsf{CAST} function. We select this operation for exclusive translation. 
Operations such as different built-in functions are typical candidates for isolation.

\paragraph{(3) Operation Extension.} For the selected operation $q_i$, if the \llm fails to translate $q_i$ within maximal trials (i.e., having parsing errors in the revised query \(Q'\)), we denote {the current operation $q_i$ as insufficient and} dynamically extend the operation to include adjacent operations that might assist the translation. This extension allows for a wide scope of translation. For example, if the \textsf{CAST} function is not successfully translated within maximal trials, we expand it to the \textsf{select\_stmt} to perform translation over a wider scope with more query operations involved.


\hi{Syntax-Augmented Translation.} 
For each identified problematic operation, we employ \llm informed by specifications via model-based syntax matching to perform translation. This ensures the translated operations are syntactically correct in the target dialect and maintain the original query's intent (functionality equivalent).

{\it (1) Model-Based Syntax Matching:} For each identified operation \(Q_i\), we employ the \dialectmodel to align syntax elements in the target dialect (see Section~\ref{subsec:train}). For instance, the \textsf{CAST} function in PostgreSQL is mapped to the \textsf{CAST} function in MySQL. 
Then, both the specifications about \textsf{CAST} function in PostgreSQL and MySQL serve as the input to instruct \llm for accurate translations.

{\it (2) Iterative LLM Translation:} Given the input SQL, its specification, and the matched specifications in the target dialect, we employ \llm (e.g., GPT-4o) to perform iterative translations. In each iteration, the \llm considers both the operation and its matched syntax elements to progressively refine the translation. 

\iffalse
This process continues until one of the following conditions is met:

$\bullet$ \bfit{Case 1:} The translated operation is syntactically valid in the target database (passes the parser) and functionally equivalent to the original operation.
    
$\bullet$ \bfit{Case 2:} The \llm determines that the target dialect cannot achieve the exact functionality due to fundamental differences (e.g., lack of specific features).

In the first case, we proceed to the following validation step. In the second case, we return to the \textit{Validation-Guided operation Selection} step to extend the current operation, potentially incorporating more parts of the query to provide additional context for translation. For example, if translating a proprietary analytical function is unsuccessful, we might include the surrounding \textsf{SELECT} clause or even consider rewriting the logic using available functions in the target dialect. \zxh{check the example}
\fi

%Given the operations together with their matched similar syntaxes in the target database, we utilize \llm to iteratively translate the operation until (1) the translated operation is both legal (by passing the target database parser) and functionally equivalent to the origin operation or (2) \llm identifies that the matched syntaxes cannot achieve the exact same functionality as the origin operation. For the former case, we enter the next step; and for the latter case, we feed back to the {\it Validation-Guided operation Selection} module to extend the scope of current operation (e.g., \zxh{add}).

{\it (3) Hybrid Query Validation:} 
We adopt a hybrid strategy to validate the translated operations.
Specifically, we employ a two-step validation mechanism to separately utilize local failures and specifications to perform syntactically correct and functionally equivalent translations.

$\bullet$ \bfit{Step 1: Syntactic Validation.} 
The translated query operations replace the identified ones to derive the translated query \(Q'\).
Then, we generate the syntax tree of \(Q'\) with the BNF definitions in the target dialect and observe whether incompatibility warnings persist.

$\bullet$ \bfit{Step 2: Semantic Validation.} 
Once the translated query \(Q'\) is syntactically correct (i.e., no incompatibility error exists), we instruct \llm to reflect whether the translation is successful.
Specifically, we provide \llm with the specifications of the identified and the translated query operations as well as the input query \(Q\) and translated query \(Q'\), instructing its reasoning about the equivalence judgment of two queries (typically easier than conduct translation). 

{Note, with the above two-step validation, we can effectively evaluate the functionality equivalence of the translated query (see Table~\ref{tab: acc}) and do not need to actually execute in the database (which generally not allowed in real scenarios).}

% \zxh{what if they take much time? sampling / limit xxx strategy?}
%\zxh{how to resolve ``same function but different result'' cases?}

\iffalse
If the revised query passes validation, the translation is considered successful. If issues arise, we repeat the translation process, refining the operation or extending its scope as necessary.

Once the revised query passes validation tests, we can terminate the translation process without examining the remaining operations. This early termination is possible since we focus on and resolve the critical areas causing parsing errors, ensuring that the incompatibilities are addressed. %By doing so, we achieve efficient translation while maintaining high accuracy.%In this way, we balance rule-based translation with the flexibility of \llms to ensure accurate and reliable query transformations.
\fi

\iffalse
\subsection{Translation Caching}  To enhance the efficiency and accuracy of future translations, we maintain a translation repository consisting of pairs of successfully translated queries that were not supported in traditional methods. Here, we generate two types of translation knowledge: \zxh{sync}

$\bullet$ \bfit{Textual Translation Hints}: Instructive descriptions that explain the mappings between functions, keywords, or syntactic constructs in the query pairs (e.g., how a specific function in the source dialect corresponds to one in the target dialect).

$\bullet$ \bfit{Executable Translation Functions}: Well-defined, rule-based functions such as regular expressions that can deterministically translate queries without further reliance on \llms.
\fi

%We maintain the informative translation knowledge base with the pairs of successfully translated queries. Specifically, we utilize LLM to generate the following translation knowledge: (1) \emph{Textual Translation Hint}: instructive descriptions (e.g., the mapping of the functions or keywords) about the query pairs; (2) \emph{Executable Translation Function}: well-formatted rule functions deterministically translate the queries without the usage of LLM (e.g., the regular expressions). We next illustrate how we generate these two types of translation knowledge.


% \zw{In-context learning, TBD}

% \zw{clarify the limitation} 

\iffalse
For the input queries, we adopt a hybrid translation strategy by first utilizing the existing rule-based translators and then LLM to translate the queries that fail to be translated by existing rules.
Besides, we employ a \zw{local-to-global} translation mechanism by first handle a series of the query operations and then whole query with the operations prepared.

These queries are divided into operations with the methods presented in Section~\ref{}.
We leverage both the \emph{syntax} and \emph{semantic} information to identify the query operations required to be translated.
For the syntax information, we rely on our implemented tree builder in Section~\ref{} to find the position raising the parsing error to locate the operations required to be translated.
For example, the tree builder will throw a message that xxx encounters the parsing error in Figure~\ref{} \zw{(same figure to be added)}.
For the semantic information, we rely on the \zxh{parser} feedback to identify the corresponding query operations (e.g., absent built-in functions in the target dialects).

For each collected query operation, we \zxh{retrieve} the top-k similar descriptions as the ones of the keyword usage in the operations (i.e., the cosine similarity of the embeddings by the model in Section~\ref{sec: embed}).
The retrieved descriptions are first\zw{re-evaluated by \llms to check whether some of these corresponding sites syntaxes can achieve the same functionality}  and compressed to be a concise representation (e.g., remove the relevant sentences or generate a \zw{summary}).
The query operations, along with the corresponding translation knowledge (i.e., the retrieved descriptions and the associated keywords), serve as the input to LLM.
Specifically, our prompt template for this task is defined as follows \zw{(TBD)}:

For the translated operations, we first separately utilize the query parser (legal) and \llm (the same functionality) to examine it.

Next, we construct the whole queries based on the translated operations by LLM (e.g., replace the corresponding subtrees with the returned ones).
Since there exists some circumstances when significant changes are required with the whole query considered (e.g., xxxx), we process the query with the translated query operations replaced, conduct extra normalization operations and let LLM to carry out global transaltion. 
If these queries are not successfully translated, we invoke LLM with additional feedback (i.e., verified by our tree builder and the database syntactically and semantically) to continue translation in an iterative manner$\footnote{Note that we define a translation failure when the tanslation rounds of each query operation in local translation stage or the whole query in the global translation stage exceed pre-defined threshold.}$.

That is, if the incompatibility warnings still occur in the operation, we extend the sagment by \zxh{add}; otherwise, we input the operation to further translate.
\fi
